Visual search and recognition for robot task execution and monitoring

Visual search of relevant targets in the environment is a crucial robot skill. We propose a preliminary framework for the execution monitor of a robot task, taking care of the robot attitude to visually searching the environment for targets involved in the task. Visual search is also relevant to recover from a failure. The framework exploits deep reinforcement learning to acquire a "common sense" scene structure and it takes advantage of a deep convolutional network to detect objects and relevant relations holding between them. The framework builds on these methods to introduce a vision-based execution monitoring, which uses classical planning as a backbone for task execution. Experiments show that with the proposed vision-based execution monitor the robot can complete simple tasks and can recover from failures in autonomy.

==> abstract.tex <==
The execution and monitoring of high-level robot actions in a real environment can be concretely enhanced addressing the problem with an hybrid deterministic/nondeterministic state machine streaming perceptual information, strengthened by visual search and recognition. The great results of deep learning allow to strongly rely on visual perception,  for both  monitoring the state of the world in terms of preconditions and postconditions that hold before and after the execution of an action and using a search policy to either guide where to look at or to refocus in case of a failure.
In this work we present an hybrid execution monitor system, which comprises a planning environment with visual search and recognition for a robot executing tasks in an uncharted environment.
This system interacts with the environment via a visual stream that uses two DCNN for recognizing the objects the robot has to deal with and manipulate, and a non- parametric Bayes estimation to discover the relations out of the DCNN features. To recover from lack of focus and failures due to missed objects we resort to visual search policies via deep reinforcement learning.

==> method.tex <==
We create an hybrid system, called visual execution monitoring (VExM), able to interact with the planning environment and the real environment. The VExM connects the two environments generating and coordinating an information flow of planning, execution, and monitoring about the current state, the executed action and the action to be executed in such a state. This information concerns objects, terms and relations mentioned in the pre and postconditions of the action.\\
Here we introduce the ``hybrid'' term because the system comprise a deterministic planner, based on FastDownward \cite{helmert-2006}, augmented with both non deterministic \emph{visual search} and visual interpretation of preconditions and postconditions of actions.

%The robot execution monitor (VExM) we consider interacts both with the planning environment and with the real world environment. It exchanges information about the current state, the executed action  and  the action to be executed in such a state. This information concerns objects, terms and relations mentioned in the pre and postconditions of the action, and it is oriented by the visual search policies.
%In order to monitor the state of execution we embed real time recognition of objects and relations which we call the \emph{visual system}, within a hybrid planning model. 

The deterministic planner is designed in PDDL. As usual, we have a \emph{domain} composed of objects, relations, real numbers and actions, which are part of the \emph{robot language}, with actions definition, specifying the preconditions and postconditions of each action.
The whole robot task is split in several goals, for each of which a \emph{problem} with initial conditions is defined. For each goal, if a plan leading from the initial state to the goal exists, then the FastDownward planner \cite{helmert-2006} infers a sequence of actions leading to the goal. The planning and ordered execution of these plans constitute the roadmap for completing the whole task.

The non deterministic part is composed of two components. The first component is the \emph{visual system}, a real time system for recognition of objects and relations designed to monitor the state of execution. The \emph{visual system} is defined by a hierarchical model combining two deep convolution neural networks (DCNN)s \cite{ren-2015} for object recognition, and a non-parametric Bayes model DPM\cite{ferguson-1973} that uses the active features of the two DCNNs to segment  the depth images collected during task execution. The combination of segmented depth and object labels allows to infer visual relations from the robot point of view. More in details, for each object $ob_j$ detected by the DCNN we estimate a statistics of the active features with dimension $38\times 50\times 512$, taken before the last pooling layer, at each pixel inside the recognized object bounding box $bb(ob_j)$. With this features set, we can estimate a more accurate depth than that available from the bounding boxes of the depth map provided by RGB-D camera. Indeed, some of the objects involved in the robot tasks, such as table, shelf, diverter, spraybottle and so on, have bounding boxes containing also other parts of the environment (see Fig. \ref{fig:train} and Fig. \ref{fig:test}).
\begin{figure}[!htb]
    \centering
    \begin{minipage}{.47\textwidth}
    \centering
        \includegraphics[width=0.95\linewidth]{figs/training}
        \caption{Training phase with the V-Rep environment}
        \label{fig:train}
    \end{minipage}%
    \begin{minipage}{0.47\textwidth}
    \centering
        \includegraphics[width=0.95\linewidth]{figs/testing}
        \caption{Testing phase in an uncharted environment}
        \label{fig:test}
    \end{minipage}
\end{figure}
This problem implies that the detection of an object returns incoherent depth and the decision for execution monitoring on controlling actions, such as \emph{grasp}, \emph{hand{-}over}, \emph{place}, \emph{open}, \emph{close} and so on, cannot take place. In order to resolve this drawback, we further elaborate the content inside the bounding boxes, classifying the content with an infinite mixture obtained by the DPM \cite{ferguson-1973}, where the inference to obtain the model is done using the Chinese Restaurant process \cite{blei-2010}, assuming that the features are realization of a normal distribution.\\

\subsection{Visual Search}
\input{methodVisSearch}
